Label Smoothing Improves Machine Unlearning

The objective of machine unlearning (MU) is to eliminate previously learned data from a model. However, it is challenging to strike a balance between computation cost and performance when using existing MU techniques. Taking inspiration from the influence of label smoothing on model confidence and differential privacy, we propose a simple gradient-based MU approach that uses an inverse process of label smoothing. This work introduces UGradSL, a simple, plug-and-play MU approach that uses smoothed labels. We provide theoretical analyses demonstrating why properly introducing label smoothing improves MU performance. We conducted extensive experiments on six datasets of various sizes and different modalities, demonstrating the effectiveness and robustness of our proposed method. The consistent improvement in MU performance is only at a marginal cost of additional computations. For instance, UGradSL improves over the gradient ascent MU baseline by 66% unlearning accuracy without sacrificing unlearning efficiency.

==> proposed_method.tex <==
\section{Negative Label Smoothing Enables Fast and Effective Unlearning}

This section sets up the analysis and shows that properly performing negative label smoothing enables fast and effective unlearning. The key ingredients of our approach are gradient ascent (GA) and label smoothing (LS). We start with understanding how GA helps with unlearning and then move on to show the power of LS. At the end of the section, we formally present our algorithm. 

\subsection{Gradient Ascent Can Help Gradient-Based Machine Unlearning}
We discuss three sets of model parameters in the MU problem: 1) $\btheta_{tr}^*$, the optimal parameters trained from $D_{tr} \sim \mathcal{D}_{tr}$ 
% \SL{why not just say $\mathcal{D}_{tr}$. Any purpose for introducing $D_{tr}$?} \zl{ Because we define $\mathcal{D}$ as the distribution of the dataset in Sec. \ref{sec:MU_def}.}
, 2) $\btheta_{r}^*$, the optimal parameters trained from $D_{r} \sim \mathcal{D}_r$, and 3) $\btheta_{f}^*$, the optimal parameters unlearned using gradient ascent (GA). 
Note $\btheta_r^*$ can be viewed as the \textit{exact} MU model. 
The definitions of $\btheta_{tr}^{*}$ and $\btheta_{r}^{*}$ are similar to Equation \ref{equ:min_erm} and by using the influence function, $\btheta_{f}^{*}$ is 
\[
    \btheta_f^{*} = \arg \min _{\btheta} R_f(\btheta) = \arg \min _{\btheta} \{R_{tr}(\btheta)+\epsilon \sum_{z^{f} \in D_{f}}\ell(h_{\btheta},z^{f})\}
\]
%With abuse of notation we will use $\sum_{i \in D}\ell(h_{\btheta},z_i}):=\sum_{i \in D} \ell(h_{\btheta},z_i)$, where $i$ denotes the $i$-the element in a dataset $D$ according to a particular order.  
where $R_{tr}(\btheta)=\sum_{z^{tr} \in D_{tr}} \ell(h_{\btheta}, z^{tr})$ is the empirical risk on $D_{tr}$. $\epsilon$ is the weight of $D_f$ compared with $D_{tr}$.
The optimal parameter can be found when the gradient is 0:
\begin{equation}
\label{equ:unlearning_opt}
    \nabla_{\btheta} R_{f}(\btheta_{f}^{*}) = \nabla_{\btheta} R_{tr}(\btheta_{f}^{*}) + \epsilon \sum_{z^{f} \in D_f}\nabla_{\btheta}\ell(h_{\btheta_{f}^{*}}, z^{f}) = 0.
\end{equation}

Expanding Eq.~(\ref{equ:unlearning_opt}) at $\btheta = \btheta_{tr}^{*}$ using the Taylor series, we have
% \begin{small}
\begin{equation}
% \tiny
% \begin{align}
\begin{split}
\label{equ:f_tr_para}
     \btheta^{*}_{f} - \btheta^{*}_{tr}  \approx -\left[\sum_{z^{tr} \in D_{tr}} \nabla_{\btheta}^{2} \ell(h_{\btheta_{tr}^{*}}, z^{tr})
     + \epsilon \sum_{z^{f} \in D_{f}}\nabla_{\btheta}^2 \ell(h_{\btheta_{tr}^{*}}, z^{f}) \right]^{-1}
    \left( \epsilon \sum_{z^{f} \in D_{f}} \nabla_{\btheta} \ell(h_{\btheta_{tr}^{*}}, z^{f})\right).
% \end{align}
\end{split}
\end{equation}

% \end{small}
% \begin{equation}
% \label{equ:f_tr_para}

% \end{equation}

Similarly, we can expand $R_{tr}(\btheta_{tr}^*)$ at $\btheta = \btheta_r^{*}$ and derive $\btheta_{r}^* - \btheta_{tr}^*$ as 
\[
    \btheta^{*}_{r} - \btheta^{*}_{tr} \approx \left(\sum_{z^{tr} \in D_{tr}} \nabla^2_{\btheta} \ell(h_{\btheta_{r}^{*}},z^{tr})\right)^{-1}\left(\sum_{z^{tr} \in 
 D_{tr}} \nabla_{\btheta} \ell(h_{\btheta_{r}^{*}}, z^{tr})\right)
\]

We ignore the average operation in the original definition of the influence function for computation convenience because the size of $D_{tr}$ or $D_f$ are fixed. 
For GA, let $\epsilon = -1$ in Equation \ref{equ:f_tr_para} and we have
\begin{equation}
\label{equ:param_distance}
\begin{split}
    \btheta_{r}^{*} - \btheta_{f}^{*} & \approx \btheta_{r}^{*} - \btheta_{tr}^{*} - (\btheta^{*}_{f} - \btheta^{*}_{tr}) = {\vec{a}}  - {\vec{b}}, \text{where}
\end{split}
\end{equation}
$\vec{a}:=(\sum_{z^{tr} \in D_{tr}} \nabla_{\btheta}^2 \ell(h_{\btheta_{r}^{*}}, z^{tr}))^{-1}\sum_{z^{tr} \in D_{tr}} \nabla_{\btheta} \ell(h_{\btheta_{r}^{*}}, z^{tr})$ and $\vec{b} := (\sum_{z^{r} \in D_r}\nabla^2_{\btheta} \ell(h_{\btheta_{tr}^{*}}, z^{r}))^{-1}\sum_{z^{f} \in D_{f}}\nabla_{\btheta} \ell(h_{\btheta^{*}_{tr}}, z^{f})$.
% {\small $$\vec{a}:=(\sum_{z^{tr} \in D_{tr}} \nabla_{\btheta}^2 \ell(h_{\btheta_{r}^{*}}, z^{tr}))^{-1}\sum_{z^{tr} \in D_{tr}} \nabla_{\btheta} \ell(h_{\btheta_{r}^{*}}, z^{tr}),~~ \vec{b} := (\sum_{z^{r} \in D_r}\nabla^2_{\btheta} \ell(h_{\btheta_{tr}^{*}}, z^{r}))^{-1}\sum_{z^{f} \in D_{f}}\nabla_{\btheta} \ell(h_{\btheta^{*}_{tr}}, z^{f})$$}%
are the \textit{true} learning phase and the \textit{backtracked} unlearning phase, respectively. In the ideal case where the inner products of first- (gradient) and second-order (Hessian) variables of $\vec{a}$ and $\vec{b}$ are the same, GA achieves exact machine unlearning since $\btheta_{r}^{*} = \btheta_{f}^{*}$. 
% \zl{$\vec{a}$ is the model difference between $\btheta_r^{*}$ and $\btheta_{tr}^{*}$ in the vector space while $\vec{b}$ is the model difference between $\btheta_f^{*}$ and $\btheta_{tr}^{*}$.}
%\zl{
Vector $(-\vec{a})$ is the Newton direction of learning $D_f$ (forget data) starting from $\btheta_r^{*}$.
% with gradient descent, meaning the difference between $\btheta_r^{*}$ and $\btheta_{tr}^*$ when the model learns $D_f$. 
Vector $\vec{b}$ is the Newton direction of unlearning $D_f$ starting from $\btheta_{tr}^{*}$.
% influence of $D_f$ on $\btheta_{tr}^{*}$ with gradient ascent, meaning the difference between $\btheta_{tr}^{*}$ and $\btheta_{f}^{*}$ when the model unlearns $D_f$.
However, in practice, due to the inconsistency between $\btheta^{*}_{tr}$ and $\btheta^{*}_{r}$, $\|\btheta_{r}^{*} - \btheta_{f}^{*}\|$ cannot be naively treated as $0$, i.e., GA cannot always help MU. We summarize it in Theorem~\ref{the:GA_helps}.
%\yl{can we add intuitions to emphasize what a,b are?}

\begin{theorem}
\label{the:GA_helps}
% There exists a $\btheta_f^*$ and we find GA can improve MU by decreasing the distance between the unlearned parameter $\btheta_f^*$ and the exact MU parameter $\btheta_r^{*}$, i.e.
Given the approximation in Equation~\ref{equ:param_distance}, GA achieves exact MU if and only if 
\[
\sum_{z^{f} \in D_{f}} \nabla_{\btheta} \ell(h_{\btheta_{r}^{*}}, z^{f}) =  - \bm H(\btheta_{r}^{*}, \btheta_{tr}^{*}) \cdot \sum_{z^{f} \in D_{f}}\nabla_{\btheta} \ell(h_{\btheta^{*}_{tr}}, z^{f}),
\]
where ${\tiny \bm H(\btheta_{r}^{*}, \btheta_{tr}^{*}) = \left(\sum_{z^{tr} \in D_{tr}} \nabla_{\btheta}^2 \ell(h_{\btheta_{r}^{*}}, z^{tr})\right) \left(\sum_{z^{r} \in D_r}\nabla^2_{\btheta} \ell(h_{\btheta_{tr}^{*}}, z^{r})\right)^{-1}}$. Otherwise, there exist $\btheta_{r}^{*}, \btheta_{tr}^{*}$ such that GA can not help MU, i.e., 
$
 \|\btheta_r^{*} - \btheta_f^{*}\| > \|\btheta_r^* - \btheta_{tr}^*\|.
$

% % We have $\left|\|\vec{a}\| - \|\vec{b}\| \right| \leq  \|\vec{a}-\vec{b}\| \leq ||\vec{a}|| + ||\vec{b}||$, indicating that $||\vec{a}-\vec{b}|| \leq ||\vec{a}||$ may or may not hold, i.e., GA cannot always help MU. 
% % Use a statement to explain the equation below, i.e.
% \begin{equation*}
%     ||\btheta_r^{*} - \btheta_f^{*}|| \leq ||\btheta_r^* - \btheta_{tr}^*||,
% \end{equation*}
% where $\btheta_{tr}^{*}$ is the optimal parameter trained with $D_{tr}$.
\end{theorem}

% From Theorem \ref{the:GA_helps}, we know GA does not always work. When the angle between $\vec{a}$ and $\vec{b}$ is larger than $\frac{\pi}{2}$, GA does not work and a more reliable method is needed.
% when GA does not work

% From Theorem \ref{the:GA_helps}, we can 
% Therefore, there exists a $\btheta_f^*$ so that we have
% \begin{equation}
%     ||\btheta_r^{*} - \btheta_f^{*}|| \leq ||\btheta_r^* - \btheta_{tr}^*||,
% \end{equation}

% meaning that GA can decrease the distance between the unlearned model and $\btheta_r^*$.
% The detailed proof is given in Appendix. 
% \begin{equation}
%     \begin{split}
%         ||||
%     \end{split}
% \end{equation}

\subsection{Negative Label Smoothing Improves MU}
\label{sec:nls_MU}

In practice, we cannot guarantee that GA always helps MU as shown in Theorem~\ref{the:GA_helps}. To alleviate the possible undesired effect of GA, we propose to use label smoothing as a plug-in module.
% Limited by the definition of loss function, $\ell$ is cross-entropy loss in the context of LS. 
Consider the cross-entropy loss as an example.
For GLS, the loss is calculated as
\begin{equation}
\begin{split}
\label{equ:gls}
    \ell(h_{\btheta}, z^{\text{GLS}, \alpha}) = \left(1+\frac{1-K}{K}\alpha\right)\cdot \ell(h_{\btheta}, (x,y)) + \frac{\alpha}{K}\sum_{y^{\prime}\in \mathcal{Y} \backslash y} \ell(h_{\btheta}, (x,y^{\prime})),
\end{split}
\end{equation}
where we use notations $\ell(h_{\btheta},  (x,y)):=\ell(h_{\btheta}, z)$ to specify the loss of an example $z=(x, y)$ in the dataset and $\ell(h_{\btheta}, (x,y))$ to denote the loss of an example when its label is replaced with $y^{\prime}$.


% When $\alpha > 0$, Equation \ref{equ:ls_cond} holds when 
% \begin{equation}
% \label{equ:rgt0}
%     \langle \nabla_{\btheta} \ell(h_{\btheta}, y), \nabla_{\btheta} \ell(h_{\btheta}, y) - \sum_{i \in \mathcal{Y} \backslash y} \nabla_{\btheta} \ell(h_{\btheta}, i) \rangle < 0
% \end{equation}

% When $\alpha < 0$, Equation \ref{equ:ls_cond} holds when
% \begin{equation}
% \label{equ:rlt0}
%     \langle \nabla_{\btheta} \ell(h_{\btheta}, y), \nabla_{\btheta} \ell(h_{\btheta}, y) - \sum_{i \in \mathcal{Y} \backslash y} \nabla_{\btheta} \ell(h_{\btheta}, i) \rangle > 0
% \end{equation}


% When we apply NLS in GA, Equation \ref{equ:param_distance} will become
% \begin{equation}
%     \btheta_{r}^{*} - \btheta_{f}^{*, NLS, \alpha} = \btheta_{r}^{*} - \btheta_{tr}^{*} - \left(\sum_{D_r}\nabla^2_{\btheta} \ell(h_{\btheta_{tr}^{*}}(z_{i}^{r}))\right)^{-1}\sum_{D_{f}}\nabla_{\btheta} \ell(h_{\btheta^{*}_{tr}}(z^{f, NLS, \alpha}_{i})),
% \end{equation}

% where $\btheta_{f}^{*, NLS, \alpha}$ is the optimal model parameter unlearned with NLS. 

\paragraph{How the smoothed term works}
Intuitively, Term $\sum_{y^{\prime} \in \mathcal{Y} \backslash y} \ell(h_{\btheta}, (x, y^{\prime}))$ leads to a state where the model makes wrong predictions on data in the forgetting dataset with equally low confidence \citep{wei2021smooth,lukasik2020does}. If the exact MU state does not overfit any points in the forgetting dataset and takes random guesses, then Term $\sum_{y^{\prime} \in \mathcal{Y} \backslash y} \ell(h_{\btheta}, (x, y^{\prime}))$ directs the model to be closer to the exact MU. On the other hand, Term $(-\sum_{y^{\prime} \in \mathcal{Y} \backslash y} \ell(h_{\btheta}, (x, y^{\prime}))$ leads to a state where the model randomly picks one wrong prediction for each data point in the forgetting dataset with high confidence \citep{sieve2020,liu2019peer}. If the exact MU state overfits the forgetting dataset with wrong labels, then Term $(- \vec{c})$ directs the model to be closer to the exact MU. Denote by $\btheta^*_{f, \text{GLS}}$ the optimal parameters unlearned using GA and NLS, and $\langle \cdot, \cdot \rangle$ the inner product of two vectors.
We show the effect of NLS in Theorem~\ref{the:negative_is_pos}.

\begin{theorem}
\label{the:negative_is_pos}
Given the approximation in Equation~\ref{equ:param_distance} and $\langle\vec{a}-\vec{b}, \vec{c}-\vec{b}\rangle \le 0$, there exists an $\alpha < 0$ such that NLS helps GA, i.e., if $\langle\vec{a}-\vec{b}, \vec{c}-\vec{b} \rangle \le 0:~ \exists \alpha < 0,~\|\btheta_{r}^{*} - \btheta_{f, \text{GLS}}^{*}\| < \|\btheta_{r}^{*} - \btheta_{f}^{*}\|$, where
% \vspace{-0.2in}
% \begin{equation*}
% {
% % \tiny

% }
% \end{equation*}
\squishlist
\item $\vec{c}:=\frac{1}{K-1}\left(\sum_{z^r \in D_r}\nabla^2_{\btheta} \ell(h_{\btheta_{tr}^{*}}, z^{r})\right)^{-1}\sum_{z^f \in D_{f}}\nabla_{\btheta}  \sum_{y^{\prime} \in \mathcal{Y} \backslash y^f} \ell(h_{\btheta_{tr}^{*}}, (x^f, y^{\prime}))$ capturing the gradient influence of the smoothed non-target label on the weight. 
\item 
% $\vec{a}-\vec{b}$ is the model difference between $\btheta_{f}^*$ and $\btheta_{r}^*$ during the unlearning process. 
$ (-\vec{a}) + \vec{b}$ is the resultant of Newton direction of learning and unlearning.
% \zzw{}{}
\item $(-\vec{c})  + \vec{b}$ is resultant of Newton direction of learning non-target labels and unlearning the target label.
% the gradient difference between the non-target labels and the target label after label smoothing is applied.
% \zzw{}{$\vec{c} + (-\vec{b})$ is the sum of gradients of learning non-target labels and unlearning the target label.}
\squishend
\end{theorem}


%\yl{the intuition for the c term should go earlier, probably right after Theorem 2. It is also a good place to remind ppl the intuition for the a,b terms}
%\zl{Done.}
% \zl{I will add this tomorrow after I finish checking the whole proof. My brain almost stops at this time...}
% With gradient ascent, we know that the constant before Term $\sum_{i \in \mathcal{Y} \backslash y} \ell(h_{\btheta}, i)$ is larger than $0$ when $\alpha < 0$, indicating that

Now we briefly discuss when the condition $\langle\vec{a}-\vec{b}, \vec{c}-\vec{b} \rangle \le 0$ holds. $\vec{c}-\vec{b}$ roughly speaking captures the effects of the smoothing term in the unlearning process. If we assume that the exact MU model is able to fully unlearn the example and outputs random predictions, vector $\vec{c}$ contributes a direction that pushes the model closer to the exact MU state, therefore reducing $||\vec{a}-\vec{b}||$ will correspond to a negative inner product between the two terms.  %In this case, the condition holds, and negative LS is positive in MU. \yl{I still don't get this. whats the intuition of a-b and c-b? why they are on the opposite direction?} For positive label smoothing, the condition should be the opposite direction, $\langle\vec{a}-\vec{b}, \vec{c}-\vec{b} \rangle \ge 0$, which is not likely to hold in practice. The gradient of the inner production is given in Appendix. 
% \begin{theorem}
% \label{the:negative_is_pos}
% % smooth rate notation
% There exists $\alpha < 0$ and $K$ to decrease the distance between the NLS-based unlearned parameter $\btheta_{f}^{*, NLS, \alpha}$ and the exact MU parameter $\btheta_{r}^{*}$, boosting the MU performance i.e. 
% % and when $||\nabla \ell(\btheta, z)|| \geq ||\nabla \ell(\btheta, z^{GLS, r})||$, 
% \begin{equation*}
%     ||\btheta_{r}^{*} - \btheta_{f}^{*, NLS, \alpha}|| < ||\btheta_{r}^{*} - \btheta_{f}^{*}||,
% \end{equation*}
% where $\btheta_{f}^{*}$ is the unlearned model using the original label. 
% \end{theorem}


% When $||\nabla \ell(\btheta, z)|| \geq ||\nabla \ell(\btheta, z^{GLS, r})||$, the upper bound of $||\btheta_{r}^{*} - \btheta_{f}^{*, GLS, r}||$ can be smaller than that of $||\btheta_{r}^{*} - \btheta_{f}^{*}||$, 
% meaning that there exist $r$ and $K$ boosting the MU performance further.

% For a well-trained model $f_{\btheta_{tr}^{*}}$, $\nabla \ell(h_{\btheta}, y)$ is ideally very small and the direction of the gradient of the target label should be different from the direction of the non-target label a lot, satisfying the condition in Equation \ref{equ:rlt0}.
% Thus, NLS is positive in MU and more general in the practical usage, which can decrease the distance between the unlearned model and the exact MU model further. 

\subsection{UGradSL: A Plug-and-Play and Gradient-Mixed MU Method}\label{sec:framework}

Compared with Retrain, Fine-Tune (FT) and GA are much more efficient as illustrated in the Experiment part in Section \ref{sec:exp_res} with comparable or better MU performance. FT and GA focus on different perspectives of MU. FT is to transfer the knowledge of the model from $D_{tr}$ to $D_{r}$ using gradient descent (GD) while GA is to remove the knowledge of $D_{f}$ from the model. 
As a plug-and-play algorithm, our method is suitable for the gradient-based methods including FT and GA. 
UGradSL is based on GA while UGradSL+ is on FT. 
Compared with UGradSL, UGradSL+ will lead to a more comprehensive result but with a larger computation cost. 

We present UGradSL and UGradSL+ in Algorithm \ref{alg:cap}. 
For UGradSL+, we first sample a batch $B_{r} = \{z_i^r:(x_i^r, y_i^r)\}_{i=1}^{n_{B_r}}$ from $D_r$ (Line 3-4).
Additionally, we sample a batch $B_{f} = \{z_i^f:(x_i^f, y_i^f)\}_{i=1}^{n_{B_f}}$ from $D_f$ where $n_{B_r} = n_{B_f}$ (Line 5).
% In each epoch, if the method is FT-based, the main dataset we use is $D_r$. Besides the sampled batch $B_{r} = \{z_i^r:(x_i^r, y_i^r)\}_{i=1}^{n_r}$, we will sample a forgetting batch $B_{f} = \{z_i^f:(x_i^f, y_i^f)\}_{i=1}^{n_f}$ from $D_f$, additionally (Line 3-6). 
It is very likely that $D_{f}$ will be iterated several times when $D_r$ is fully iterated once because $n_r > n_f$ in general. Then we apply NLS on $B_{f}$ leading to $B_{f}^{\text{NLS}, \alpha}=\{z_i^{f, \text{NLS}, \alpha}:(x_i^f, y_i^{f, \text{NLS}, \alpha})\}$. 
% \yl{let's use text in these notations $B_{f}^{\text{NLS}, \alpha}$} \zl{Done.}
We calculate the loss using a gradient-mixed method as:
% \vspace{-0.0989cm}
\begin{equation}
\label{equ:loss_calculation}
\begin{split}
    L(h_{\btheta}, B_{f}^{\text{NLS}, \alpha}, B_{r}, p) = p \cdot \sum_{z^r \in B_r} \ell(h_{\btheta}, z^r) - (1-p) \cdot \sum_{z^{f, \text{NLS}, \alpha} \in B_f^{\text{NLS}, \alpha}} \ell(h_{\btheta}, z^{f, \text{NLS}, \alpha}),
\end{split}
\end{equation}
where $p \in [0, 1]$ is used to balance GD and GA and the minus sign stands for the GA. $h_{\btheta}$ is updated according to $L$ (Line 6).
UGradSL is similar to UGradSL+ and the dataset used is given in bracket in Algorithm \ref{alg:cap}.
The difference between UGradSL and UGradSL+ is the convergence standard.
% \yl{what's the difference in the convergence standard?} \zl{I added a convergence before $D_r$ and $D_f$.} 
UGradSL is based on the convergence of $D_f$ while UGradSL+ is based on $D_r$.
It should be noted that the Hessian matrix in Theorem \ref{the:GA_helps} is only used in the theoretical proof. In the practical calculation, \textbf{there is no need to calculate the Hessian matrix}. 
Thus, our method does not incur substantially more computation but improves the MU performance on a large scale. We present empirical evidence in Section \ref{sec:exp_res}. 
One of the concerns using influence function is the convexity. 
All the analysis is based on the converged or the almost converged model weights. 
For example, the loss landscape of $\btheta^{*}_{tr}$ is given in the Appendix \ref{sec:loss_landscape}.
% Because UGradSL+ usually needs more iterations, UGradSL+ is slower than UGradSL but with a more comprehensive 


% The GA-based algorithm is similar to FT-based (Line 9-12). Because FT-based method usually needs more iteration, FT-based method is slower than GA-based. Compared with the original GA and FT, 

\begin{algorithm}
\caption{UGradSL+: A plug-and-play, efficient, gradient-based MU method using NLS. UGradSL can be specified by imposing the  {\color{blue} dataset replacement} in the bracket. 
% The pink background stands for the \colorbox{MistyRose1}{FT-based} method while the yellow background stands for the \colorbox{PaleGreen1}{GA-based}, showing the plug-and-play characteristic of this method in the gradient-based method.
}
\label{alg:cap}
\begin{algorithmic}[1]
\Require A almost-converged model $h_{\hat{\btheta}_{tr}}$ trained with $D_{tr}$. The retained dataset $D_r$. The forgetting dataset $D_f$. The smoothing rate $\alpha$. Unlearning epochs $E$. GA ratio $p$.
\Ensure The unlearned model $h_{\btheta_f}$.
\State Set the current epoch index as $t_c \gets 1$

% \State $y \gets 1$
% \State $X \gets x$
% \State $N \gets n$
% TODO: Propose the most complex algoritm, highlight NLS
\While{$t_c < E$}
% \If{\colorbox{MistyRose1}{FT-based}} \Comment{Mini-batch updating and the iteration time depends on $D_{r}$.}
%     % \State $X \gets X \times X$
%     % \State $N \gets \frac{N}{2}$  \Comment{This is a comment}
    \While{{$D_{r} ({\color{blue}D_{f}})$ is not fully iterated}} 
    % \Comment{Use $\mathcal{D}_f$ instead of $\mathcal{D}_{tr}$ for UGradSL}
    \State {Sample a batch $B_{r}$ in $D_{r}$}
    \State {Sample a batch $B_{f}$ from $D_{f}$ where the size of $B_{f}$ is the same as that of $B_{r}$}
    \State Update the model using $B_{r}$, $B_{f}$, $p$ and $\alpha$ according to Equation \ref{equ:loss_calculation}
    \EndWhile
% \ElsIf{\colorbox{PaleGreen1}{GA-based}} \Comment{Mini-batch updating and the iteration time depends on $D_{f}$.}
% \While{\colorbox{PaleGreen1}{$D_{f}$ is not fully iterated}} 
%     \State \colorbox{PaleGreen1}{Sample a batch $B_{f}$ in $D_{f}$}
%     \State \colorbox{PaleGreen1}{Sample a batch $B_{tr}$ from $D_{tr}$ where the size of $B_{tr}$ is the same as that of $B_{f}$}
%     \State Update the model using $B_{tr}$, $B_{f}$, $p$ and $\alpha$ according to Equation \ref{equ:loss_calculation}
%     \EndWhile
% \EndIf
\State $t_c \gets t_c + 1$
\EndWhile
\end{algorithmic}
\end{algorithm}
